OGLE-BLAP-009 -- A Case Study for the Properties and Evolution of Blue Large-Amplitude Pulsators

Blue large-amplitude pulsators (BLAPs) make up a rare class of hot pulsating stars with effective temperatures of $\approx$30,000 K and surface gravities of 4.0 - 5.0 dex (cgs). The evolutionary origin and current status of BLAPs is not well understood, largely based on a lack of spectroscopic observations and no available mass constraints. However, several theoretical models have been proposed that reproduce their observed properties, including studies that identify them as pulsating helium-core pre-white dwarfs (He-core pre-WDs). We present here follow-up high-speed photometry and phase-resolved spectroscopy of one of the original 14 BLAPs, OGLE-BLAP-009, discovered during the Optical Gravitational Lensing Experiment. We aim to explore its pulsation characteristics and determine stellar properties such as mass and radius in order to test the consistency of these results with He-core pre-WD models. Using the mean atmospheric parameters found using spectroscopy, we fit a spectral energy distribution to obtain a preliminary estimate of the radius, luminosity and mass by making use of the Gaia parallax. We then compare the consistency of these results to He-core pre-WD models generated using MESA, with predicted pulsation periods implemented using GYRE. We find that our mass constraints are in agreement with a low-mass He-core pre-WD of $\approx$0.30 M$_{\odot}$.

==> BIB.tex <==
%______________________________________________________
% INTRO________________________________________________
%______________________________________________________
@ARTICLE{irrgang2013,
       author = {{Irrgang}, A. and {Wilcox}, B. and {Tucker}, E. and {Schiefelbein}, L.},
        title = "{Milky Way mass models for orbit calculations}",
      journal = {\aap},
     keywords = {dark matter, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = jan,
       volume = {549},
          eid = {A137},
        pages = {A137},
          doi = {10.1051/0004-6361/201220540},
archivePrefix = {arXiv},
       eprint = {1211.4353},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...549A.137I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tmts_blap,
       author = {{Lin}, Jie and {Wu}, Chengyuan and {Wang}, Xiaofeng and {N{\'e}meth}, P{\'e}ter and {Xiong}, Heran and {Wu}, Tao and {Filippenko}, Alexei V. and {Cai}, Yongzhi and {Brink}, Thomas G. and {Yan}, Shengyu and {Zeng}, Xiangyun and {Luo}, Yangping and {Xiang}, Danfeng and {Zhang}, Jujia and {Zheng}, WeiKang and {Yang}, Yi and {Mo}, Jun and {Xi}, Gaobo and {Zhang}, Jicheng and {Iskandar}, Abdusamatjan and {Esamdin}, Ali and {Jiang}, Xiaojun and {Sai}, Hanna and {Wei}, Zixuan and {Chen}, Liyang and {Guo}, Fangzhou and {Chen}, Zhihao and {Li}, Wenxiong and {Lin}, Weili and {Lin}, Han and {Zhang}, Xinghan},
        title = "{An 18.9 min blue large-amplitude pulsator crossing the `Hertzsprung gap' of hot subdwarfs}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = feb,
       volume = {7},
        pages = {223-233},
          doi = {10.1038/s41550-022-01783-z},
archivePrefix = {arXiv},
      eprint = {2209.06617},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023NatAs...7..223L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaiadr3var,
       author = {{Rimoldini}, Lorenzo and {Holl}, Berry and {Gavras}, Panagiotis and {Audard}, Marc and {De Ridder}, Joris and {Mowlavi}, Nami and {Nienartowicz}, Krzysztof and {Jevardat de Fombelle}, Gr{\'e}gory and {Lecoeur-Ta{\"\i}bi}, Isabelle and {Karbevska}, Lea and {Evans}, Dafydd W. and {{\'A}brah{\'a}m}, P{\'e}ter and {Carnerero}, Maria I. and {Clementini}, Gisella and {Distefano}, Elisa and {Garofalo}, Alessia and {Garc{\'\i}a-Lario}, Pedro and {Gomel}, Roy and {Klioner}, Sergei A. and {Kruszy{\'n}ska}, Katarzyna and {Lanzafame}, Alessandro C. and {Lebzelter}, Thomas and {Marton}, G{\'a}bor and {Mazeh}, Tsevi and {Molinaro}, Roberto and {Panahi}, Aviad and {Raiteri}, Claudia M. and {Ripepi}, Vincenzo and {Szabados}, L{\'a}szl{\'o} and {Teyssier}, David and {Trabucchi}, Michele and {Wyrzykowski}, {\L}ukasz and {Zucker}, Shay and {Eyer}, Laurent},
        title = "{Gaia Data Release 3: All-sky classification of 12.4 million variable sources into 25 classes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = nov,
          eid = {arXiv:2211.17238},
        pages = {arXiv:2211.17238},
          doi = {10.48550/arXiv.2211.17238},
archivePrefix = {arXiv},
       eprint = {2211.17238},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv221117238R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gaia,
       author = {{Gaia Collaboration} and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Brown}, A.~G.~A. and {Vallenari}, A. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Milligan}, D.~J. and {Panem}, C. and {Poinsignon}, V. and {Pourbaix}, D. and {Randich}, S. and {Sarri}, G. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {Valette}, V. and {van Leeuwen}, F. and {Walton}, N.~A. and {Aerts}, C. and {Arenou}, F. and {Cropper}, M. and {Drimmel}, R. and {H{\o}g}, E. and {Katz}, D. and {Lattanzi}, M.~G. and {O'Mullane}, W. and {Grebel}, E.~K. and {Holland}, A.~D. and {Huc}, C. and {Passot}, X. and {Bramante}, L. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Hern{\'a}ndez}, J. and {Jean-Antoine-Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Panuzzo}, P. and {Portell}, J. and {Richards}, P.~J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Torra}, J. and {Els}, S.~G. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Lock}, T. and {Mercier}, E. and {Altmann}, M. and {Andrae}, R. and {Astraatmadja}, T.~L. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Cowell}, S. and {Creevey}, O. and {Cuypers}, J. and {Davidson}, M. and {De Ridder}, J. and {de Torres}, A. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fr{\'e}mat}, Y. and {Garc{\'\i}a-Torres}, M. and {Gosset}, E. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hauser}, M. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Huckle}, H.~E. and {Hutton}, A. and {Jasniewicz}, G. and {Jordan}, S. and {Kontizas}, M. and {Korn}, A.~J. and {Lanzafame}, A.~C. and {Manteiga}, M. and {Moitinho}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Smith}, K.~W. and {Sozzetti}, A. and {Thuillot}, W. and {van Reeven}, W. and {Viala}, Y. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aguado}, J.~J. and {Allan}, P.~M. and {Allasia}, W. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Ant{\'o}n}, S. and {Arcay}, B. and {Atzei}, A. and {Ayache}, L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Barache}, C. and {Barata}, C. and {Barbier}, A. and {Barblan}, F. and {Baroni}, M. and {Barrado y Navascu{\'e}s}, D. and {Barros}, M. and {Barstow}, M.~A. and {Becciani}, U. and {Bellazzini}, M. and {Bellei}, G. and {Bello Garc{\'\i}a}, A. and {Belokurov}, V. and {Bendjoya}, P. and {Berihuete}, A. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Billebaud}, F. and {Blagorodnova}, N. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and {Bourda}, G. and {Bouy}, H. and {Bragaglia}, A. and {Breddels}, M.~A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Bucciarelli}, B. and {Budnik}, F. and {Burgess}, P. and {Burgon}, R. and {Burlacu}, A. and {Busonero}, D. and {Buzzi}, R. and {Caffau}, E. and {Cambras}, J. and {Campbell}, H. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carlucci}, T. and {Carrasco}, J.~M. and {Castellani}, M. and {Charlot}, P. and {Charnas}, J. and {Charvet}, P. and {Chassat}, F. and {Chiavassa}, A. and {Clotet}, M. and {Cocozza}, G. and {Collins}, R.~S. and {Collins}, P. and {Costigan}, G. and {Crifo}, F. and {Cross}, N.~J.~G. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {De Cat}, P. and {de Felice}, F. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {di Marco}, F. and {Di Matteo}, P. and {Diakite}, S. and {Distefano}, E. and {Dolding}, C. and {Dos Anjos}, S. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Dzigan}, Y. and {Ecale}, E. and {Edvardsson}, B. and {Enke}, H. and {Erdmann}, M. and {Escolar}, D. and {Espina}, M. and {Evans}, N.~W. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Faye}, F. and {Federici}, L. and {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fouesneau}, M. and {Fraile}, E. and {Fraser}, M. and {Fuchs}, J. and {Furnell}, R. and {Gai}, M. and {Galleti}, S. and {Galluccio}, L. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Gar{\'e}}, P. and {Garofalo}, A. and {Garralda}, N. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guerrier}, A. and {Guillout}, P. and {Guiraud}, J. and {G{\'u}rpide}, A. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Haigron}, R. and {Hatzidimitriou}, D. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Hobbs}, D. and {Hofmann}, W. and {Holl}, B. and {Holland}, G. and {Hunt}, J.~A.~S. and {Hypki}, A. and {Icardi}, V. and {Irwin}, M. and {Jevardat de Fombelle}, G. and {Jofr{\'e}}, P. and {Jonker}, P.~G. and {Jorissen}, A. and {Julbe}, F. and {Karampelas}, A. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Koubsky}, P. and {Kowalczyk}, A. and {Krone-Martins}, A. and {Kudryashova}, M. and {Kull}, I. and {Bachchan}, R.~K. and {Lacoste-Seris}, F. and {Lanza}, A.~F. and {Lavigne}, J. -B. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lemaitre}, V. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\"o}ffler}, W. and {L{\'o}pez}, M. and {Lopez-Lozano}, A. and {Lorenz}, D. and {Loureiro}, T. and {MacDonald}, I. and {Magalh{\~a}es Fernandes}, T. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marie}, J. and {Marinoni}, S. and {Marrese}, P.~M. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Mart{\'\i}n-Fleitas}, J.~M. and {Martino}, M. and {Mary}, N. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Mestre}, A. and {Michalik}, D. and {Millar}, N.~R. and {Miranda}, B.~M.~H. and {Molina}, D. and {Molinaro}, R. and {Molinaro}, M. and {Moln{\'a}r}, L. and {Moniez}, M. and {Montegriffo}, P. and {Monteiro}, D. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and {Morley}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Narbonne}, J. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {Ord{\'e}novic}, C. and {Ordieres-Mer{\'e}}, J. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Parsons}, P. and {Paulsen}, T. and {Pecoraro}, M. and {Pedrosa}, R. and {Pentik{\"a}inen}, H. and {Pereira}, J. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Ragaini}, S. and {Rago}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Ranalli}, P. and {Rauw}, G. and {Read}, A. and {Regibo}, S. and {Renk}, F. and {Reyl{\'e}}, C. and {Ribeiro}, R.~A. and {Rimoldini}, L. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rudolph}, A. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sarasso}, M. and {Savietto}, H. and {Schnorhk}, A. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {Segransan}, D. and {Serpell}, E. and {Shih}, I. -C. and {Smareglia}, R. and {Smart}, R.~L. and {Smith}, C. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Tingley}, B. and {Trager}, S.~C. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Valentini}, G. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Varadi}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Via}, T. and {Vicente}, D. and {Vogt}, S. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Weingrill}, K. and {Werner}, D. and {Wevers}, T. and {Whitehead}, G. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T. and {Alecu}, A. and {Allen}, M. and {Allende Prieto}, C. and {Amorim}, A. and {Anglada-Escud{\'e}}, G. and {Arsenijevic}, V. and {Azaz}, S. and {Balm}, P. and {Beck}, M. and {Bernstein}, H. -H. and {Bigot}, L. and {Bijaoui}, A. and {Blasco}, C. and {Bonfigli}, M. and {Bono}, G. and {Boudreault}, S. and {Bressan}, A. and {Brown}, S. and {Brunet}, P. -M. and {Bunclark}, P. and {Buonanno}, R. and {Butkevich}, A.~G. and {Carret}, C. and {Carrion}, C. and {Chemin}, L. and {Ch{\'e}reau}, F. and {Corcione}, L. and {Darmigny}, E. and {de Boer}, K.~S. and {de Teodoro}, P. and {de Zeeuw}, P.~T. and {Delle Luche}, C. and {Domingues}, C.~D. and {Dubath}, P. and {Fodor}, F. and {Fr{\'e}zouls}, B. and {Fries}, A. and {Fustes}, D. and {Fyfe}, D. and {Gallardo}, E. and {Gallegos}, J. and {Gardiol}, D. and {Gebran}, M. and {Gomboc}, A. and {G{\'o}mez}, A. and {Grux}, E. and {Gueguen}, A. and {Heyrovsky}, A. and {Hoar}, J. and {Iannicola}, G. and {Isasi Parache}, Y. and {Janotto}, A. -M. and {Joliet}, E. and {Jonckheere}, A. and {Keil}, R. and {Kim}, D. -W. and {Klagyivik}, P. and {Klar}, J. and {Knude}, J. and {Kochukhov}, O. and {Kolka}, I. and {Kos}, J. and {Kutka}, A. and {Lainey}, V. and {LeBouquin}, D. and {Liu}, C. and {Loreggia}, D. and {Makarov}, V.~V. and {Marseille}, M.~G. and {Martayan}, C. and {Martinez-Rubi}, O. and {Massart}, B. and {Meynadier}, F. and {Mignot}, S. and {Munari}, U. and {Nguyen}, A. -T. and {Nordlander}, T. and {Ocvirk}, P. and {O'Flaherty}, K.~S. and {Olias Sanz}, A. and {Ortiz}, P. and {Osorio}, J. and {Oszkiewicz}, D. and {Ouzounis}, A. and {Palmer}, M. and {Park}, P. and {Pasquato}, E. and {Peltzer}, C. and {Peralta}, J. and {P{\'e}turaud}, F. and {Pieniluoma}, T. and {Pigozzi}, E. and {Poels}, J. and {Prat}, G. and {Prod'homme}, T. and {Raison}, F. and {Rebordao}, J.~M. and {Risquez}, D. and {Rocca-Volmerange}, B. and {Rosen}, S. and {Ruiz-Fuertes}, M.~I. and {Russo}, F. and {Sembay}, S. and {Serraller Vizcaino}, I. and {Short}, A. and {Siebert}, A. and {Silva}, H. and {Sinachopoulos}, D. and {Slezak}, E. and {Soffel}, M. and {Sosnowska}, D. and {Strai{\v{z}}ys}, V. and {ter Linden}, M. and {Terrell}, D. and {Theil}, S. and {Tiede}, C. and {Troisi}, L. and {Tsalmantza}, P. and {Tur}, D. and {Vaccari}, M. and {Vachier}, F. and {Valles}, P. and {Van Hamme}, W. and {Veltz}, L. and {Virtanen}, J. and {Wallut}, J. -M. and {Wichmann}, R. and {Wilkinson}, M.~I. and {Ziaeepour}, H. and {Zschocke}, S.},
        title = "{The Gaia mission}",
      journal = {\aap},
     keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = nov,
       volume = {595},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201629272},
archivePrefix = {arXiv},
       eprint = {1609.04153},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...595A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gaiadr3,
       author = {{Gaia Collaboration} and {Vallenari}, A. and {Brown}, A.~G.~A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Arenou}, F. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Ducourant}, C. and {Evans}, D.~W. and {Eyer}, L. and {Guerra}, R. and {Hutton}, A. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U.~L. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Tanga}, P. and {Walton}, N.~A. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Drimmel}, R. and {Jansen}, F. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Guerrier}, A. and {Heiter}, U. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo{\o}rcit}, R. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P.~W. and {Busonero}, D. and {Busso}, G. and {C{\'a}novas}, H. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {de Teodoro}, P. and {Nu{\~n}ez Campos}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Esquej}, P. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fraile}, E. and {Garabato}, D. and {Garc{\'\i}a-Lario}, P. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Recio-Blanco}, A. and {Reyl{\'e}}, C. and {Riello}, M. and {Rimoldini}, L. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {Abbas}, U. and {{\'A}brah{\'a}m}, P. and {Abreu Aramburu}, A. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Aldea-Montero}, F. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and {Anders}, F. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Binnenfeld}, A. and {Blanco-Cuaresma}, S. and {Blazere}, A. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiaramida}, V. and {Chiavassa}, A. and {Chornay}, N. and {Comoretto}, G. and {Contursi}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Cropper}, M. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delisle}, J. -B. and {Demouchy}, C. and {Dharmawardena}, T.~E. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Edvardsson}, B. and {Enke}, H. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fournier}, Y. and {Fouron}, C. and {Fragkoudi}, F. and {Gai}, M. and {Garcia-Gutierrez}, A. and {Garcia-Reinaldos}, M. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavel}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Santamar{\'\i}a}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guillout}, P. and {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Helmer}, A. and {Helmi}, A. and {Sarmiento}, M.~H. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jardine}, K. and {Jasniewicz}, G. and {Jean-Antoine Piccolo}, A. and {Jim{\'e}nez-Arranz}, {\'O}. and {Jorissen}, A. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {K{\'o}sp{\'a}l}, {\'A} and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Kun}, M. and {Laizeau}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E.~L. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Lorca}, A. and {Loup}, C. and {Madrero Pardo}, P. and {Magdaleno Romeo}, A. and {Managau}, S. and {Mann}, R.~G. and {Manteiga}, M. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos}, J. and {Marcos Santos}, M.~M.~S. and {Mar{\'\i}n Pina}, D. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Polo}, L. Martin and {Mart{\'\i}n-Fleitas}, J.~M. and {Marton}, G. and {Mary}, N. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Monari}, G. and {Mongui{\'o}}, M. and {Montegriffo}, P. and {Montero}, A. and {Mor}, R. and {Mora}, A. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Nagy}, Z. and {Noval}, L. and {Oca{\~n}a}, F. and {Ogden}, A. and {Ordenovic}, C. and {Osinde}, J.~O. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Pallas-Quintela}, L. and {Panahi}, A. and {Payne-Wardenaar}, S. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Pichon}, B. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Richards}, P.~J. and {Rios Diaz}, C. and {Ripepi}, V. and {Riva}, A. and {Rix}, H. -W. and {Rixon}, G. and {Robichon}, N. and {Robin}, A.~C. and {Robin}, C. and {Roelens}, M. and {Rogues}, H.~R.~O. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruz Mieres}, D. and {Rybicki}, K.~A. and {Sadowski}, G. and {S{\'a}ez N{\'u}{\~n}ez}, A. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Silvelo}, A. and {Slezak}, E. and {Slezak}, I. and {Smart}, R.~L. and {Snaith}, O.~N. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spina}, L. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Taylo}, M.~B. and {Teixeira}, R. and {Tolomei}, L. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Torralba Elipe}, G. and {Trabucchi}, M. and {Tsounis}, A.~T. and {Turon}, C. and {Ulla}, A. and {Unger}, N. and {Vaillant}, M.~V. and {van Dillen}, E. and {van Reeven}, W. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, L. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zwitter}, T.},
        title = "{Gaia Data Release 3: Summary of the content and survey properties}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jul,
          eid = {arXiv:2208.00211},
        pages = {arXiv:2208.00211},
          doi = {10.48550/arXiv.2208.00211},
archivePrefix = {arXiv},
       eprint = {2208.00211},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220800211G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Macfarlane_2017,
       author = {{Macfarlane}, S.~A. and {Woudt}, P.~A. and {Groot}, P.~J. and {Ramsay}, G. and {Toma}, R. and {Motsoaledi}, M. and {Crause}, L.~A. and {Gilbank}, D.~G. and {O'Donoghue}, D. and {Potter}, S.~B. and {Sickafoose}, A.~A. and {van Gend}, C. and {Worters}, H.~L.},
        title = "{The OmegaWhite survey for short-period variable stars - III: follow-up photometric and spectroscopic observations}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: observational, techniques: photometric, surveys, binaries: close, Galaxy: bulge, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = feb,
       volume = {465},
       number = {1},
        pages = {434-459},
          doi = {10.1093/mnras/stw2704},
archivePrefix = {arXiv},
       eprint = {1610.05687},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465..434M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{BLAPDISC2017,
       author = {{Pietrukowicz}, Pawe{\l} and {Dziembowski}, Wojciech A. and {Latour}, Marilyn and {Angeloni}, Rodolfo and {Poleski}, Rados{\l}aw and {di Mille}, Francesco and {Soszy{\'n}ski}, Igor and {Udalski}, Andrzej and {Szyma{\'n}ski}, Micha{\l} K. and {Wyrzykowski}, {\L}ukasz and {Koz{\l}owski}, Szymon and {Skowron}, Jan and {Skowron}, Dorota and {Mr{\'o}z}, Przemek and {Pawlak}, Micha{\l} and {Ulaczyk}, Krzysztof},
        title = "{Blue large-amplitude pulsators as a new class of variable stars}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = aug,
       volume = {1},
          eid = {0166},
        pages = {0166},
          doi = {10.1038/s41550-017-0166},
archivePrefix = {arXiv},
       eprint = {1706.07802},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017NatAs...1E.166P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CHeB_ev,
       author = {{Wu}, Tao and {Li}, Yan},
        title = "{Which evolutionary status does the Blue Large-Amplitude Pulsators stay at?}",
      journal = {\mnras},
     keywords = {asteroseismology, stars: evolution, stars: interiors, stars: oscillations, pulsars: individual: BLAPs, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = aug,
       volume = {478},
       number = {3},
        pages = {3871-3877},
          doi = {10.1093/mnras/sty1347},
archivePrefix = {arXiv},
       eprint = {1805.07073},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.478.3871W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SHeB_ev,
       author = {{Xiong}, H. and {Casagrande}, L. and {Chen}, X. and {Vos}, J. and {Zhang}, X. and {Justham}, S. and {Li}, J. and {Wu}, T. and {Li}, Y. and {Han}, Z.},
        title = "{Shell helium-burning hot subdwarf B stars as candidates for blue large-amplitude pulsators}",
      journal = {\aap},
     keywords = {binaries: general, stars: oscillations, subdwarfs, stars: peculiar, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = dec,
       volume = {668},
          eid = {A112},
        pages = {A112},
          doi = {10.1051/0004-6361/202244571},
archivePrefix = {arXiv},
       eprint = {2211.01564},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...668A.112X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bryne_2018,
       author = {{Byrne}, Conor M. and {Jeffery}, C. Simon},
        title = "{Post-common envelope binary stars, radiative levitation, and blue large-amplitude pulsators}",
      journal = {\mnras},
     keywords = {diffusion, stars: evolution, stars: oscillations, stars: horizontal branch, subdwarfs, white dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = dec,
       volume = {481},
       number = {3},
        pages = {3810-3820},
          doi = {10.1093/mnras/sty2545},
archivePrefix = {arXiv},
       eprint = {1809.04183},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.481.3810B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Byrne_2020,
       author = {{Byrne}, Conor M. and {Jeffery}, C. Simon},
        title = "{Pulsation in faint blue stars}",
      journal = {\mnras},
     keywords = {diffusion, stars: evolution, stars: oscillations, subdwarfs, white dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = feb,
       volume = {492},
       number = {1},
        pages = {232-244},
          doi = {10.1093/mnras/stz3486},
archivePrefix = {arXiv},
       eprint = {1912.04129},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492..232B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Byrne_2021,
       author = {{Byrne}, C.~M. and {Stanway}, E.~R. and {Eldridge}, J.~J.},
        title = "{Binary evolution pathways of blue large-amplitude pulsators}",
      journal = {\mnras},
     keywords = {methods: numerical, binaries: general, stars: evolution, stars: oscillations, white dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = oct,
       volume = {507},
       number = {1},
        pages = {621-631},
          doi = {10.1093/mnras/stab2115},
archivePrefix = {arXiv},
       eprint = {2107.14628},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.507..621B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meng_2020,
       author = {{Meng}, Xiang-Cun and {Han}, Zhan-Wen and {Podsiadlowski}, Philipp and {Li}, Jiao},
        title = "{Blue Large-amplitude Pulsators: The Possible Surviving Companions of Type Ia Supernovae}",
      journal = {\apj},
     keywords = {Type Ia supernovae, White dwarf stars, Variable stars, Supernova remnants, 1728, 1799, 1761, 1667, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = nov,
       volume = {903},
       number = {2},
          eid = {100},
        pages = {100},
          doi = {10.3847/1538-4357/abbb8e},
archivePrefix = {arXiv},
       eprint = {2009.11059},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...903..100M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Romero_2018,
       author = {{Romero}, Alejandra D. and {C{\'o}rsico}, A.~H. and {Althaus}, L.~G. and {Pelisoli}, I. and {Kepler}, S.~O.},
        title = "{On the evolutionary status and pulsations of the recently discovered blue large-amplitude pulsators (BLAPs)}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: variables: general, white dwarf, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = jun,
       volume = {477},
       number = {1},
        pages = {L30-L34},
          doi = {10.1093/mnrasl/sly051},
archivePrefix = {arXiv},
       eprint = {1803.09600},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477L..30R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cors_2016,
       author = {{C{\'o}rsico}, A.~H. and {Althaus}, L.~G. and {Serenelli}, A.~M. and {Kepler}, S.~O. and {Jeffery}, C.~S. and {Corti}, M.~A.},
        title = "{Pulsating low-mass white dwarfs in the frame of new evolutionary sequences. III. The pre-ELM white dwarf instability strip}",
      journal = {\aap},
     keywords = {asteroseismology, stars: oscillations, stars: evolution, stars: interiors, white dwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = apr,
       volume = {588},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201528032},
archivePrefix = {arXiv},
       eprint = {1602.03195},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...588A..74C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cors_ev,
       author = {{C{\'o}rsico}, Alejandro H. and {Romero}, Alejandra D. and {Althaus}, Leandro G. and {Pelisoli}, Ingrid and {Kepler}, S.~O.},
        title = "{Blue Large-Amplitude Pulsators (BLAPs): possible origin, evolutionary status, and nature of their pulsations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = sep,
          eid = {arXiv:1809.07451},
        pages = {arXiv:1809.07451},
          doi = {10.48550/arXiv.1809.07451},
archivePrefix = {arXiv},
       eprint = {1809.07451},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv180907451C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kupfer_2019,
       author = {{Kupfer}, Thomas and {Bauer}, Evan B. and {Burdge}, Kevin B. and {Bellm}, Eric C. and {Bildsten}, Lars and {Fuller}, Jim and {Hermes}, JJ and {Kulkarni}, Shrinivas R. and {Prince}, Thomas A. and {van Roestel}, Jan and {Dekany}, Richard and {Duev}, Dmitry A. and {Feeney}, Michael and {Giomi}, Matteo and {Graham}, Matthew J. and {Kaye}, Stephen and {Laher}, Russ R. and {Masci}, Frank J. and {Porter}, Michael and {Riddle}, Reed and {Shupe}, David L. and {Smith}, Roger M. and {Soumagnac}, Maayane T. and {Szkody}, Paula and {Ward}, Charlotte},
        title = "{A New Class of Large-amplitude Radial-mode Hot Subdwarf Pulsators}",
      journal = {\apjl},
     keywords = {asteroseismology, stars: oscillations, stars: variables: general, white dwarfs, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {878},
       number = {2},
          eid = {L35},
        pages = {L35},
          doi = {10.3847/2041-8213/ab263c},
archivePrefix = {arXiv},
       eprint = {1906.00979},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...878L..35K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ramsay_2022,
       author = {{Ramsay}, Gavin and {Woudt}, Patrick A. and {Kupfer}, Thomas and {van Roestel}, Jan and {Paterson}, Kerry and {Warner}, Brian and {Buckley}, David A.~H. and {Groot}, Paul J. and {Heber}, Ulrich and {Irrgang}, Andreas and {Jeffery}, C. Simon and {Motsoaledi}, Mokhine and {Schwartz}, Martinus J. and {Wevers}, Thomas},
        title = "{The OmegaWhite survey for short-period variable stars - VII. High amplitude short-period blue variables}",
      journal = {\mnras},
     keywords = {astronomical data bases: surveys, binaries, stars: oscillations, stars: variable, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jun,
       volume = {513},
       number = {2},
        pages = {2215-2225},
          doi = {10.1093/mnras/stac1000},
archivePrefix = {arXiv},
       eprint = {2204.03265},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.513.2215R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McWhirter_2022,
       author = {{McWhirter}, Paul Ross and {Lam}, Marco C.},
        title = "{Identifying blue large amplitude pulsators from Gaia DR2 and ZTF DR3}",
      journal = {\mnras},
     keywords = {methods: data analysis, stars: early-type, stars: oscillations, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = apr,
       volume = {511},
       number = {4},
        pages = {4971-4980},
          doi = {10.1093/mnras/stac291},
archivePrefix = {arXiv},
       eprint = {2201.11862},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511.4971M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heber_1986,
       author = {{Heber}, U.},
        title = "{The atmosphere of subluminous B stars. II. Analysis of 10 helium poor subdwarfs and the birthrate of sdB stars.}",
      journal = {\aap},
     keywords = {B Stars, Horizontal Branch Stars, Stellar Atmospheres, Stellar Evolution, Stellar Spectra, Subdwarf Stars, Abundance, Diffusion, Interstellar Extinction, Statistical Analysis, Stellar Gravitation, Stellar Luminosity, Stellar Temperature, Ultraviolet Spectra, White Dwarf Stars, Astrophysics},
         year = 1986,
        month = jan,
       volume = {155},
        pages = {33-45},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986A&A...155...33H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heber_2009,
       author = {{Heber}, Ulrich},
        title = "{Hot Subdwarf Stars}",
      journal = {\araa},
         year = 2009,
        month = sep,
       volume = {47},
       number = {1},
        pages = {211-251},
          doi = {10.1146/annurev-astro-082708-101836},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ARA&A..47..211H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heber_2016,
       author = {{Heber}, U.},
        title = "{Hot Subluminous Stars}",
      journal = {\pasp},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = aug,
       volume = {128},
       number = {966},
        pages = {082001},
          doi = {10.1088/1538-3873/128/966/082001},
archivePrefix = {arXiv},
       eprint = {1604.07749},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PASP..128h2001H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{OGLE4,
       author = {{Udalski}, A. and {Szyma{\'n}ski}, M.~K. and {Szyma{\'n}ski}, G.},
        title = "{OGLE-IV: Fourth Phase of the Optical Gravitational Lensing Experiment}",
      journal = {\actaa},
     keywords = {Surveys, Techniques: Photometric, Galaxy: bulge, Galaxy: disk, Magellanic Clouds, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = mar,
       volume = {65},
       number = {1},
        pages = {1-38},
archivePrefix = {arXiv},
       eprint = {1504.05966},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AcA....65....1U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%______________________________________________________
% OBSERVATIONS_________________________________________
%______________________________________________________


@ARTICLE{ESI,
       author = {{Sheinis}, A.~I. and {Bolte}, M. and {Epps}, H.~W. and {Kibrick}, R.~I. and {Miller}, J.~S. and {Radovan}, M.~V. and {Bigelow}, B.~C. and {Sutin}, B.~M.},
        title = "{ESI, a New Keck Observatory Echellette Spectrograph and Imager}",
      journal = {\pasp},
     keywords = {Instrumentation: Spectrographs, Techniques: Spectroscopic, Astrophysics},
         year = 2002,
        month = aug,
       volume = {114},
       number = {798},
        pages = {851-865},
          doi = {10.1086/341706},
archivePrefix = {arXiv},
       eprint = {astro-ph/0204297},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002PASP..114..851S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LRIS,
       author = {{Oke}, J.~B. and {Cohen}, J.~G. and {Carr}, M. and {Cromer}, J. and {Dingizian}, A. and {Harris}, F.~H. and {Labrecque}, S. and {Lucinio}, R. and {Schaal}, W. and {Epps}, H. and {Miller}, J.},
        title = "{The Keck Low-Resolution Imaging Spectrometer}",
      journal = {\pasp},
     keywords = {INSTRUMENTATION: SPECTROGRAPHS},
         year = 1995,
        month = apr,
       volume = {107},
        pages = {375},
          doi = {10.1086/133562},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995PASP..107..375O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{per19,
   author = {{Perley}, D.~A.},
    title = "{Fully-Automated Reduction of Longslit Spectroscopy with the Low Resolution Imaging Spectrometer at Keck Observatory}",
  journal = {arXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1903.07629},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2019,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190307629P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Robin2003,
       author = {{Robin}, A.~C. and {Reyl{\'e}}, C. and {Derri{\`e}re}, S. and {Picaud}, S.},
        title = "{A synthetic view on structure and evolution of the Milky Way}",
      journal = {\aap},
     keywords = {Galaxy: stellar content, Galaxy: general, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: structure},
         year = 2003,
        month = oct,
       volume = {409},
        pages = {523-540},
          doi = {10.1051/0004-6361:20031117},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...409..523R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%______________________________________________________
% PHOTOMETRY___________________________________________
%______________________________________________________
@ARTICLE{monoperiod,
       author = {{McWhirter}, Paul Ross and {Lam}, Marco C. and {Steele}, Iain A.},
        title = "{Confirmation of monoperiodicity above 20 s for two blue large-amplitude pulsators}",
      journal = {\mnras},
     keywords = {stars: white dwarfs, stars: oscillations, stars: variables: general, methods: data analysis, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {496},
       number = {2},
        pages = {1105-1114},
          doi = {10.1093/mnras/staa1560},
archivePrefix = {arXiv},
       eprint = {2006.03346},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.1105M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{P04,
       author = {{Lenz}, P. and {Breger}, M.},
        title = "{Period04 User Guide}",
      journal = {Communications in Asteroseismology},
         year = 2005,
        month = jun,
       volume = {146},
        pages = {53-136},
          doi = {10.1553/cia146s53},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005CoAst.146...53L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gaia_2018,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Bailer-Jones}, C.~A.~L. and {Biermann}, M. and {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and {van Leeuwen}, F. and {Walton}, N.~A. and {Arenou}, F. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and {Guerra}, R. and {Holl}, B. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nienartowicz}, K. and {Panuzzo}, P. and {Portell}, J. and {Riello}, M. and {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Audard}, M. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Burgess}, P. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Clementini}, G. and {Clotet}, M. and {Creevey}, O. and {Davidson}, M. and {De Ridder}, J. and {Delchambre}, L. and {Dell'Oro}, A. and {Ducourant}, C. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Galluccio}, L. and {Garc{\'\i}a-Torres}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gonz{\'a}lez-Vidal}, J.~J. and {Gosset}, E. and {Guy}, L.~P. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Hutton}, A. and {Jasniewicz}, G. and {Jean-Antoine-Piccolo}, A. and {Jordan}, S. and {Korn}, A.~J. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {L{\"o}ffler}, W. and {Manteiga}, M. and {Marrese}, P.~M. and {Mart{\'\i}n-Fleitas}, J.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Rimoldini}, L. and {Robin}, A.~C. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {S{\"u}veges}, M. and {Torra}, J. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alvarez}, R. and {Alves}, J. and {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and {Antiche}, E. and {Antoja}, T. and {Arcay}, B. and {Astraatmadja}, T.~L. and {Bach}, N. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balm}, P. and {Barache}, C. and {Barata}, C. and {Barbato}, D. and {Barblan}, F. and {Barklem}, P.~S. and {Barrado}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartholom{\'e} Mu{\~n}oz}, S. and {Bassilana}, J. -L. and {Becciani}, U. and {Bellazzini}, M. and {Berihuete}, A. and {Bertone}, S. and {Bianchi}, L. and {Bienaym{\'e}}, O. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Boeche}, C. and {Bombrun}, A. and {Borrachero}, R. and {Bossini}, D. and {Bouquillon}, S. and {Bourda}, G. and {Bragaglia}, A. and {Bramante}, L. and {Breddels}, M.~A. and {Bressan}, A. and {Brouillet}, N. and {Br{\"u}semeister}, T. and {Brugaletta}, E. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {Cannizzaro}, G. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cocozza}, G. and {Costigan}, G. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Cuypers}, J. and {Dafonte}, C. and {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {de Martino}, D. and {de Souza}, R. and {de Torres}, A. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Drazinos}, P. and {Dur{\'a}n}, J. and {Edvardsson}, B. and {Enke}, H. and {Eriksson}, K. and {Esquej}, P. and {Eynard Bontemps}, G. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and {Farr{\`a}s Casas}, M. and {Federici}, L. and {Fedorets}, G. and {Fernique}, P. and {Figueras}, F. and {Filippi}, F. and {Findeisen}, K. and {Fonti}, A. and {Fraile}, E. and {Fraser}, M. and {Fr{\'e}zouls}, B. and {Gai}, M. and {Galleti}, S. and {Garabato}, D. and {Garc{\'\i}a-Sedano}, F. and {Garofalo}, A. and {Garralda}, N. and {Gavel}, A. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Glass}, F. and {Gomes}, M. and {Granvik}, M. and {Gueguen}, A. and {Guerrier}, A. and {Guiraud}, J. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Haigron}, R. and {Hatzidimitriou}, D. and {Hauser}, M. and {Haywood}, M. and {Heiter}, U. and {Helmi}, A. and {Heu}, J. and {Hilger}, T. and {Hobbs}, D. and {Hofmann}, W. and {Holland}, G. and {Huckle}, H.~E. and {Hypki}, A. and {Icardi}, V. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jonker}, P.~G. and {Juh{\'a}sz}, {\'A}. L. and {Julbe}, F. and {Karampelas}, A. and {Kewley}, A. and {Klar}, J. and {Kochoska}, A. and {Kohley}, R. and {Kolenberg}, K. and {Kontizas}, M. and {Kontizas}, E. and {Koposov}, S.~E. and {Kordopatis}, G. and {Kostrzewa-Rutkowska}, Z. and {Koubsky}, P. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Lavigne}, J. -B. and {Le Fustec}, Y. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Lenhardt}, H. and {Leroux}, F. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {L{\'o}pez}, M. and {Managau}, S. and {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and {Marchant}, J.~M. and {Marconi}, M. and {Marinoni}, S. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and {Martino}, M. and {Marton}, G. and {Mary}, N. and {Massari}, D. and {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and {Musella}, I. and {Nelemans}, G. and {Nicastro}, L. and {Noval}, L. and {O'Mullane}, W. and {Ord{\'e}novic}, C. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and {Palacin}, H. and {Palaversa}, L. and {Panahi}, A. and {Pawlak}, M. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rambaux}, N. and {Ramos-Lerate}, M. and {Regibo}, S. and {Reyl{\'e}}, C. and {Riclet}, F. and {Ripepi}, V. and {Riva}, A. and {Rivard}, A. and {Rixon}, G. and {Roegiers}, T. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Ruiz-Dern}, L. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Sanna}, N. and {Santana-Ros}, T. and {Sarasso}, M. and {Savietto}, H. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Shih}, I. -C. and {Siltala}, L. and {Silva}, A.~F. and {Smart}, R.~L. and {Smith}, K.~W. and {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {Stoev}, H. and {Suess}, F.~F. and {Surdej}, J. and {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Terrett}, D. and {Teyssandier}, P. and {Thuillot}, W. and {Titarenko}, A. and {Torra Clotet}, F. and {Turon}, C. and {Ulla}, A. and {Utrilla}, E. and {Uzzi}, S. and {Vaillant}, M. and {Valentini}, G. and {Valette}, V. and {van Elteren}, A. and {Van Hemelryck}, E. and {van Leeuwen}, M. and {Vaschetto}, M. and {Vecchiato}, A. and {Veljanoski}, J. and {Viala}, Y. and {Vicente}, D. and {Vogt}, S. and {von Essen}, C. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and {Walmsley}, G. and {Weiler}, M. and {Wertz}, O. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Ziaeepour}, H. and {Zorec}, J. and {Zschocke}, S. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Data Release 2. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, techniques: radial velocities, stars: fundamental parameters, stars: variables: general, minor planets, asteroids: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = aug,
       volume = {616},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201833051},
archivePrefix = {arXiv},
       eprint = {1804.09365},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...616A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gaia_EDR3,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, techniques: radial velocities, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202039657},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%______________________________________________________
% SPECTROSCOPY_________________________________________
%______________________________________________________

@ARTICLE{nap04a,
   author = {{Napiwotzki}, R. and {Karl}, C.~A. and {Lisker}, T. and {Heber}, U. and 
	{Christlieb}, N. and {Reimers}, D. and {Nelemans}, G. and {Homeier}, D.
	},
    title = "{Close binary EHB stars from SPY}",
  journal = {Astrophysics and Space Science},
   eprint = {arXiv:astro-ph/0401201},
 keywords = {stars:, horizontal branch, evolution, binaries},
     year = 2004,
    month = jun,
   volume = 291,
    pages = {321-328},
      doi = {10.1023/B:ASTR.0000044362.07416.6c},
   adsurl = {http://adsabs.harvard.edu/abs/2004Ap%26SS.291..321N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}}

@ARTICLE{gei11a,
   author = {{Geier}, S. and {Hirsch}, H. and {Tillich}, A. and {Maxted}, P.~F.~L. and 
	{Bentley}, S.~J. and {{\O}stensen}, R.~H. and {Heber}, U. and 
	{G{\"a}nsicke}, B.~T. and {Marsh}, T.~R. and {Napiwotzki}, R. and 
	{Barlow}, B.~N. and {O'Toole}, S.~J.},
    title = "{The MUCHFUSS project - searching for hot subdwarf binaries with massive unseen companions. Survey, target selection and atmospheric parameters}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1103.4045},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: spectroscopic, subdwarfs},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A28},
    pages = {A28},
      doi = {10.1051/0004-6361/201015316},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A..28G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}}

@ARTICLE{hub17,
       author = {{Hubeny}, Ivan and {Lanz}, Thierry},
        title = "{A brief introductory guide to TLUSTY and SYNSPEC}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jun,
          eid = {arXiv:1706.01859},
        pages = {arXiv:1706.01859},
archivePrefix = {arXiv},
       eprint = {1706.01859},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017arXiv170601859H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dorsch2021,
       author = {{Dorsch}, M. and {Jeffery}, C.~S. and {Irrgang}, A. and {Woolf}, V. and {Heber}, U.},
        title = "{EC 22536{\ensuremath{-}}5304: a lead-rich and metal-poor long-period binary}",
      journal = {\aap},
     keywords = {stars: abundances, stars: chemically peculiar, subdwarfs, stars: individual: EC 22536-5304, binaries: spectroscopic, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = sep,
       volume = {653},
          eid = {A120},
        pages = {A120},
          doi = {10.1051/0004-6361/202141381},
archivePrefix = {arXiv},
       eprint = {2107.06340},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...653A.120D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dor22,
       author = {{Dorsch}, M. and {Reindl}, N. and {Pelisoli}, I. and {Heber}, U. and {Geier}, S. and {Istrate}, A.~G. and {Justham}, S.},
        title = "{Discovery of a highly magnetic He-sdO star from a double-degenerate binary merger}",
      journal = {A\&A},
     keywords = {stars: magnetic field, subdwarfs, stars: early-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = feb,
       volume = {658},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/202142880},
archivePrefix = {arXiv},
       eprint = {2201.08146},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...658L...9D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barlow_2010,
       author = {{Barlow}, B.~N. and {Dunlap}, B.~H. and {Clemens}, J.~C. and {Lynas-Gray}, A.~E. and {Ivarsen}, K.~M. and {Lacluyze}, A.~P. and {Reichart}, D.~E. and {Haislip}, J.~B. and {Nysewander}, M.~C.},
        title = "{Photometry and spectroscopy of the new sdBV CS 1246}",
      journal = {\mnras},
     keywords = {stars: individual: CS 1246, stars: oscillations, subdwarfs, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = mar,
       volume = {403},
       number = {1},
        pages = {324-334},
          doi = {10.1111/j.1365-2966.2009.16119.x},
archivePrefix = {arXiv},
       eprint = {0912.3903},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.403..324B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{projection_effect,
       author = {{Monta{\~n}{\'e}s Rodriguez}, P. and {Jeffery}, C.~S.},
        title = "{Projection effects in the spectra of early-type pulsating stars}",
      journal = {\aap},
     keywords = {STARS: EARLY-TYPE, STARS: PULSATIONS, STARS: ATMOSPHERES},
         year = 2001,
        month = aug,
       volume = {375},
        pages = {411-418},
          doi = {10.1051/0004-6361:20010840},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...375..411M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
%______________________________________________________
% DISCUSSION___________________________________________
%______________________________________________________

@ARTICLE{Baade_1926,
       author = {{Baade}, W.},
        title = "{{\"U}ber eine M{\"o}glichkeit, die Pulsationstheorie der {\ensuremath{\delta}} Cephei-Ver{\"a}nderlichen zu pr{\"u}ten}",
      journal = {Astronomische Nachrichten},
         year = 1926,
        month = oct,
       volume = {228},
       number = {20},
        pages = {359},
          doi = {10.1002/asna.19262282003},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1926AN....228..359B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wesselink_1946,
       author = {{Wesselink}, A.~J.},
        title = "{The observations of brightness, colour and radial velocity of {\ensuremath{\delta}} Cephei and the pulsation hypothesis (Errata: 10 258, 310)}",
      journal = {\bain},
         year = 1946,
        month = jan,
       volume = {10},
        pages = {91},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1946BAN....10...91W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mesa2011,
       author = {{Paxton}, Bill and {Bildsten}, Lars and {Dotter}, Aaron and {Herwig}, Falk and {Lesaffre}, Pierre and {Timmes}, Frank},
        title = "{Modules for Experiments in Stellar Astrophysics (MESA)}",
      journal = {\apjs},
     keywords = {methods: numerical, stars: evolution, stars: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jan,
       volume = {192},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.1088/0067-0049/192/1/310.48550/arXiv.1009.1622},
archivePrefix = {arXiv},
       eprint = {1009.1622},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..192....3P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mesa2013,
       author = {{Paxton}, Bill and {Cantiello}, Matteo and {Arras}, Phil and {Bildsten}, Lars and {Brown}, Edward F. and {Dotter}, Aaron and {Mankovich}, Christopher and {Montgomery}, M.~H. and {Stello}, Dennis and {Timmes}, F.~X. and {Townsend}, Richard},
        title = "{Modules for Experiments in Stellar Astrophysics (MESA): Planets, Oscillations, Rotation, and Massive Stars}",
      journal = {\apjs},
     keywords = {asteroseismology, methods: numerical, planets and satellites: physical evolution, stars: evolution, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2013,
        month = sep,
       volume = {208},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.1088/0067-0049/208/1/410.48550/arXiv.1301.0319},
archivePrefix = {arXiv},
       eprint = {1301.0319},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..208....4P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mesa2015,
       author = {{Paxton}, Bill and {Marchant}, Pablo and {Schwab}, Josiah and {Bauer}, Evan B. and {Bildsten}, Lars and {Cantiello}, Matteo and {Dessart}, Luc and {Farmer}, R. and {Hu}, H. and {Langer}, N. and {Townsend}, R.~H.~D. and {Townsley}, Dean M. and {Timmes}, F.~X.},
        title = "{Modules for Experiments in Stellar Astrophysics (MESA): Binaries, Pulsations, and Explosions}",
      journal = {\apjs},
     keywords = {binaries: general, methods: numerical, nuclear reactions, nucleosynthesis, abundances, shock waves, stars: evolution, stars: oscillations, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.1088/0067-0049/220/1/1510.48550/arXiv.1506.03146},
archivePrefix = {arXiv},
       eprint = {1506.03146},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220...15P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mesa2018,
       author = {{Paxton}, Bill and {Schwab}, Josiah and {Bauer}, Evan B. and {Bildsten}, Lars and {Blinnikov}, Sergei and {Duffell}, Paul and {Farmer}, R. and {Goldberg}, Jared A. and {Marchant}, Pablo and {Sorokina}, Elena and {Thoul}, Anne and {Townsend}, Richard H.~D. and {Timmes}, F.~X.},
        title = "{Modules for Experiments in Stellar Astrophysics (MESA): Convective Boundaries, Element Diffusion, and Massive Star Explosions}",
      journal = {\apjs},
     keywords = {convection, diffusion, hydrodynamics, methods: numerical, stars: evolution, supernovae: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = feb,
       volume = {234},
       number = {2},
          eid = {34},
        pages = {34},
          doi = {10.3847/1538-4365/aaa5a810.48550/arXiv.1710.08424},
archivePrefix = {arXiv},
       eprint = {1710.08424},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..234...34P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mesa2019,
       author = {{Paxton}, Bill and {Smolec}, R. and {Schwab}, Josiah and {Gautschy}, A. and {Bildsten}, Lars and {Cantiello}, Matteo and {Dotter}, Aaron and {Farmer}, R. and {Goldberg}, Jared A. and {Jermyn}, Adam S. and {Kanbur}, S.~M. and {Marchant}, Pablo and {Thoul}, Anne and {Townsend}, Richard H.~D. and {Wolf}, William M. and {Zhang}, Michael and {Timmes}, F.~X.},
        title = "{Modules for Experiments in Stellar Astrophysics (MESA): Pulsating Variable Stars, Rotation, Convective Boundaries, and Energy Conservation}",
      journal = {\apjs},
     keywords = {stars: evolution, stars: general, stars: interiors, stars: oscillations:  including pulsations, stars: rotation, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jul,
       volume = {243},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.3847/1538-4365/ab2241},
archivePrefix = {arXiv},
       eprint = {1903.01426},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..243...10P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gyre,
       author = {{Townsend}, R.~H.~D. and {Teitler}, S.~A.},
        title = "{GYRE: an open-source stellar oscillation code based on a new Magnus Multiple Shooting scheme}",
      journal = {\mnras},
     keywords = {methods: numerical, stars: evolution, stars: interiors, stars: oscillations, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = nov,
       volume = {435},
       number = {4},
        pages = {3406-3418},
          doi = {10.1093/mnras/stt153310.48550/arXiv.1308.2965},
archivePrefix = {arXiv},
       eprint = {1308.2965},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.435.3406T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jeffery_2015,
       author = {{Jeffery}, C.~S. and {Kurtz}, D. and {Shibahashi}, H. and {Starling}, R.~L.~C. and {Elkin}, V. and {Monta{\~n}{\'e}s-Rodr{\'\i}guez}, P. and {McCormac}, J.},
        title = "{Subaru and Swift observations of V652 Herculis: resolving the photospheric pulsation}",
      journal = {\mnras},
     keywords = {shock waves, techniques: radial velocities, stars: atmospheres, stars: chemically peculiar, stars: individual: V652 Her, stars: oscillations, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = mar,
       volume = {447},
       number = {3},
        pages = {2836-2851},
          doi = {10.1093/mnras/stu2654},
archivePrefix = {arXiv},
       eprint = {1412.8672},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.447.2836J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jeffery2022,
       author = {{Jeffery}, C. Simon},
        title = "{Spectrum synthesis for radially pulsating stars with shocked atmospheres}",
      journal = {\mnras},
     keywords = {hydrodynamics, line: profiles, radiative transfer, shock waves, stars: individual: V652 Her, stars: oscillations, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = sep,
       volume = {515},
       number = {1},
        pages = {716-729},
          doi = {10.1093/mnras/stac1644},
archivePrefix = {arXiv},
       eprint = {2206.05094},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.515..716J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jeffery_etal_2022,
       author = {{Jeffery}, C. Simon and {Monta{\~n}{\'e}s-Rodr{\'\i}guez}, Pilar and {Saio}, Hideyuki},
        title = "{Improved hydrodynamic pulsation models for the pulsating extreme helium star V652 Herculis}",
      journal = {\mnras},
     keywords = {hydrodynamics, shock waves, stars: chemically peculiar, stars: individual (V652 Her), stars: oscillations, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jan,
       volume = {509},
       number = {2},
        pages = {1940-1958},
          doi = {10.1093/mnras/stab2876},
archivePrefix = {arXiv},
       eprint = {2110.00427},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.509.1940J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Woolf_2002,
       author = {{Woolf}, V.~M. and {Jeffery}, C.~S.},
        title = "{Temperature and gravity of the pulsating extreme helium star <ASTROBJ>LSS 3184</ASTROBJ> (<ASTROBJ>BX Cir</ASTROBJ>) through its pulsation cycle}",
      journal = {\aap},
     keywords = {stars: chemically peculiar, stars: oscillations, stars: variables, stars: individual: LSS 3184, stars: atmospheres, Astrophysics},
         year = 2002,
        month = nov,
       volume = {395},
        pages = {535-540},
          doi = {10.1051/0004-6361:20021113},
archivePrefix = {arXiv},
       eprint = {astro-ph/0208269},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...395..535W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PHDTHESIS{spas,
       author = {{Hirsch}, Heiko Andreas},
        title = "{Hot subluminous stars : on the search for chemical signatures of their genesis}",
       school = {Friedrich Alexander University of Erlangen-Nuremberg, Germany},
         year = 2009,
        month = oct,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009PhDT.......273H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HD13_2022,
       author = {{Pigulski}, A. and {Kotysz}, K. and {Ko{\l}aczek-Szyma{\'n}ski}, P.~A.},
        title = "{HD 133729: A blue large-amplitude pulsator in orbit around a main-sequence B-type star}",
      journal = {\aap},
     keywords = {stars: oscillations, binaries: spectroscopic, stars: fundamental parameters, stars: individual: HD 133729, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jul,
       volume = {663},
          eid = {A62},
        pages = {A62},
          doi = {10.1051/0004-6361/202243293},
archivePrefix = {arXiv},
       eprint = {2203.11789},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...663A..62P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gast_2008,
       author = {{Gastine}, T. and {Dintrans}, B.},
        title = "{Direct numerical simulations of the {\ensuremath{\kappa}}-mechanism. II. Nonlinear saturation and the Hertzsprung progression}",
      journal = {\aap},
     keywords = {hydrodynamics, instabilities, waves, stars: oscillations, stars: variables: Cepheids, methods: numerical, Astrophysics},
         year = 2008,
        month = nov,
       volume = {490},
       number = {2},
        pages = {743-752},
          doi = {10.1051/0004-6361:200809891},
archivePrefix = {arXiv},
       eprint = {0804.0345},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...490..743G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%______________________________________________________
% CONCLUSION___________________________________________
%______________________________________________________



%_______________________________________________________

@ARTICLE{PS1_DR2,
       author = {{Magnier}, Eugene. A. and {Schlafly}, Edward. F. and {Finkbeiner}, Douglas P. and {Tonry}, J.~L. and {Goldman}, B. and {R{\"o}ser}, S. and {Schilbach}, E. and {Casertano}, S. and {Chambers}, K.~C. and {Flewelling}, H.~A. and {Huber}, M.~E. and {Price}, P.~A. and {Sweeney}, W.~E. and {Waters}, C.~Z. and {Denneau}, L. and {Draper}, P.~W. and {Hodapp}, K.~W. and {Jedicke}, R. and {Kaiser}, N. and {Kudritzki}, R. -P. and {Metcalfe}, N. and {Stubbs}, C.~W. and {Wainscoat}, R.~J.},
        title = "{Pan-STARRS Photometric and Astrometric Calibration}",
      journal = {\apjs},
     keywords = {Photometry, CCD photometry, Astrometry, Surveys, Sky surveys, Flux calibration, Proper motions, Astronomy databases, 1234, 208, 80, 1671, 1464, 544, 1295, 83, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = nov,
       volume = {251},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4365/abb82a},
archivePrefix = {arXiv},
       eprint = {1612.05242},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJS..251....6M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{VVV_DR4,
       author = {{Minniti}, D. and {Lucas}, P.~W. and {Emerson}, J.~P. and {Saito}, R.~K. and {Hempel}, M. and {Pietrukowicz}, P. and {Ahumada}, A.~V. and {Alonso}, M.~V. and {Alonso-Garcia}, J. and {Arias}, J.~I. and {Bandyopadhyay}, R.~M. and {Barb{\'a}}, R.~H. and {Barbuy}, B. and {Bedin}, L.~R. and {Bica}, E. and {Borissova}, J. and {Bronfman}, L. and {Carraro}, G. and {Catelan}, M. and {Clari{\'a}}, J.~J. and {Cross}, N. and {de Grijs}, R. and {D{\'e}k{\'a}ny}, I. and {Drew}, J.~E. and {Fari{\~n}a}, C. and {Feinstein}, C. and {Fern{\'a}ndez Laj{\'u}s}, E. and {Gamen}, R.~C. and {Geisler}, D. and {Gieren}, W. and {Goldman}, B. and {Gonzalez}, O.~A. and {Gunthardt}, G. and {Gurovich}, S. and {Hambly}, N.~C. and {Irwin}, M.~J. and {Ivanov}, V.~D. and {Jord{\'a}n}, A. and {Kerins}, E. and {Kinemuchi}, K. and {Kurtev}, R. and {L{\'o}pez-Corredoira}, M. and {Maccarone}, T. and {Masetti}, N. and {Merlo}, D. and {Messineo}, M. and {Mirabel}, I.~F. and {Monaco}, L. and {Morelli}, L. and {Padilla}, N. and {Palma}, T. and {Parisi}, M.~C. and {Pignata}, G. and {Rejkuba}, M. and {Roman-Lopes}, A. and {Sale}, S.~E. and {Schreiber}, M.~R. and {Schr{\"o}der}, A.~C. and {Smith}, M. and {}, L. Sodr{\'e}, Jr. and {Soto}, M. and {Tamura}, M. and {Tappert}, C. and {Thompson}, M.~A. and {Toledo}, I. and {Zoccali}, M. and {Pietrzynski}, G.},
        title = "{VISTA Variables in the Via Lactea (VVV): The public ESO near-IR variability survey of the Milky Way}",
      journal = {\na},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = jul,
       volume = {15},
       number = {5},
        pages = {433-443},
          doi = {10.1016/j.newast.2009.12.002},
archivePrefix = {arXiv},
       eprint = {0912.1056},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010NewA...15..433M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{UKIDSS_gps6,
       author = {{Lucas}, P.~W. and {Hoare}, M.~G. and {Longmore}, A. and {Schr{\"o}der}, A.~C. and {Davis}, C.~J. and {Adamson}, A. and {Bandyopadhyay}, R.~M. and {de Grijs}, R. and {Smith}, M. and {Gosling}, A. and {Mitchison}, S. and {G{\'a}sp{\'a}r}, A. and {Coe}, M. and {Tamura}, M. and {Parker}, Q. and {Irwin}, M. and {Hambly}, N. and {Bryant}, J. and {Collins}, R.~S. and {Cross}, N. and {Evans}, D.~W. and {Gonzalez-Solares}, E. and {Hodgkin}, S. and {Lewis}, J. and {Read}, M. and {Riello}, M. and {Sutorius}, E.~T.~W. and {Lawrence}, A. and {Drew}, J.~E. and {Dye}, S. and {Thompson}, M.~A.},
        title = "{The UKIDSS Galactic Plane Survey}",
      journal = {\mnras},
     keywords = {methods: data analysis, surveys, circumstellar matter, stars: formation, Galaxy: stellar content, Astrophysics},
         year = 2008,
        month = nov,
       volume = {391},
       number = {1},
        pages = {136-163},
          doi = {10.1111/j.1365-2966.2008.13924.x},
archivePrefix = {arXiv},
       eprint = {0712.0100},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.391..136L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DECaPS_DR1,
       author = {{Schlafly}, E.~F. and {Green}, G.~M. and {Lang}, D. and {Daylan}, T. and {Finkbeiner}, D.~P. and {Lee}, A. and {Meisner}, A.~M. and {Schlegel}, D. and {Valdes}, F.},
        title = "{The DECam Plane Survey: Optical Photometry of Two Billion Objects in the Southern Galactic Plane}",
      journal = {\apjs},
     keywords = {catalogs, surveys, techniques: photometric, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = feb,
       volume = {234},
       number = {2},
          eid = {39},
        pages = {39},
          doi = {10.3847/1538-4365/aaa3e2},
archivePrefix = {arXiv},
       eprint = {1710.01309},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..234...39S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gaia_phot, 
       author = {{Riello}, M. and {De Angeli}, F. and {Evans}, D.~W. and {Montegriffo}, P. and {Carrasco}, J.~M. and {Busso}, G. and {Palaversa}, L. and {Burgess}, P.~W. and {Diener}, C. and {Davidson}, M. and {Rowell}, N. and {Fabricius}, C. and {Jordi}, C. and {Bellazzini}, M. and {Pancino}, E. and {Harrison}, D.~L. and {Cacciari}, C. and {van Leeuwen}, F. and {Hambly}, N.~C. and {Hodgkin}, S.~T. and {Osborne}, P.~J. and {Altavilla}, G. and {Barstow}, M.~A. and {Brown}, A.~G.~A. and {Castellani}, M. and {Cowell}, S. and {De Luise}, F. and {Gilmore}, G. and {Giuffrida}, G. and {Hidalgo}, S. and {Holland}, G. and {Marinoni}, S. and {Pagani}, C. and {Piersimoni}, A.~M. and {Pulone}, L. and {Ragaini}, S. and {Rainer}, M. and {Richards}, P.~J. and {Sanna}, N. and {Walton}, N.~A. and {Weiler}, M. and {Yoldas}, A.},
        title = "{Gaia Early Data Release 3. Photometric content and validation}",
      journal = {\aap},
     keywords = {catalogs, surveys, instrumentation: photometers, techniques: photometric, Galaxy: general, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A3},
        pages = {A3},
          doi = {10.1051/0004-6361/202039587},
archivePrefix = {arXiv},
       eprint = {2012.01916},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...3R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SkyMapper_DR2,
       author = {{Onken}, Christopher A. and {Wolf}, Christian and {Bessell}, Michael S. and {Chang}, Seo-Won and {Da Costa}, Gary S. and {Luvaul}, Lance C. and {Mackey}, Dougal and {Schmidt}, Brian P. and {Shao}, Li},
        title = "{SkyMapper Southern Survey: Second data release (DR2)}",
      journal = {\pasa},
     keywords = {catalogues, methods: observational, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = aug,
       volume = {36},
          eid = {e033},
        pages = {e033},
          doi = {10.1017/pasa.2019.27},
archivePrefix = {arXiv},
       eprint = {2008.10359},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASA...36...33O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Lindegren21,
   title={Gaia Early Data Release 3},
   volume={649},
   ISSN={1432-0746},
   url={http://dx.doi.org/10.1051/0004-6361/202039653},
   DOI={10.1051/0004-6361/202039653},
   journal={\aap},
   publisher={EDP Sciences},
   author={Lindegren, L. and Bastian, U. and Biermann, M. and Bombrun, A. and de Torres, A. and Gerlach, E. and Geyer, R. and Hernández, J. and Hilger, T. and Hobbs, D. and et al.},
   year={2021},
   month={Apr},
   pages={A4}
}

@ARTICLE{Heber2018,
   author = {{Heber}, U. and {Irrgang}, A. and {Schaffenroth}, J.},
    title = "{Spectral energy distributions and colours of hot subluminous stars}",
  journal = {Open Astronomy},
archivePrefix = "arXiv",
   eprint = {1712.06546},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early type, subdwarfs, Techniques: potometric},
     year = 2018,
    month = feb,
   volume = 27,
    pages = {35-43},
      doi = {10.1515/astro-2018-0008},
   adsurl = {http://adsabs.harvard.edu/abs/2018OAst...27...35H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fitzpatrick2019,
       author = {{Fitzpatrick}, E.~L. and {Massa}, Derck and {Gordon}, Karl D. and {Bohlin}, Ralph and {Clayton}, Geoffrey C.},
        title = "{An Analysis of the Shapes of Interstellar Extinction Curves. VII. Milky Way Spectrophotometric Optical-through-ultraviolet Extinction and Its R-dependence}",
      journal = {\apj},
     keywords = {Interstellar dust, Interstellar dust extinction, Interstellar dust processes, Interstellar absorption, Interstellar reddening, Interstellar scattering, 836, 837, 838, 831, 853, 854, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {886},
       number = {2},
          eid = {108},
        pages = {108},
          doi = {10.3847/1538-4357/ab4c3a},
archivePrefix = {arXiv},
       eprint = {1910.08852},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886..108F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{El-Badry2021,
       author = {{El-Badry}, Kareem and {Rix}, Hans-Walter and {Heintz}, Tyler M.},
        title = "{A million binaries from Gaia eDR3: sample selection and validation of Gaia parallax uncertainties}",
      journal = {\mnras},
     keywords = {methods: statistical, catalogues, parallaxes, binaries: visual, stars: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = sep,
       volume = {506},
       number = {2},
        pages = {2269-2295},
          doi = {10.1093/mnras/stab323},
archivePrefix = {arXiv},
       eprint = {2101.05282},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.506.2269E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{projection_2007,
       author = {{Nardetto}, N. and {Mourard}, D. and {Mathias}, Ph. and {Fokin}, A. and {Gillet}, D.},
        title = "{High-resolution spectroscopy for Cepheids distance determination. II. A period-projection factor relation}",
      journal = {\aap},
     keywords = {techniques: spectroscopic, stars: atmospheres, stars: oscillations (including pulsations), stars: variables: Cepheids, stars: distances, Astrophysics},
         year = 2007,
        month = aug,
       volume = {471},
       number = {2},
        pages = {661-669},
          doi = {10.1051/0004-6361:20066853},
archivePrefix = {arXiv},
       eprint = {0804.1331},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...471..661N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{projection_2013,
       author = {{Guiglion}, G. and {Nardetto}, N. and {Mathias}, P. and {Domiciano de Souza}, A. and {Poretti}, E. and {Rainer}, M. and {Fokin}, A. and {Mourard}, D. and {Gieren}, W.},
        title = "{Understanding the dynamical structure of pulsating stars: The Baade-Wesselink projection factor of the {\ensuremath{\delta}} Scuti stars AI Velorum and {\ensuremath{\beta}} Cassiopeiae}",
      journal = {\aap},
     keywords = {stars: oscillations, stars: atmospheres, stars: variables:{\ensuremath{\delta}}Scuti, techniques: spectroscopic, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2013,
        month = feb,
       volume = {550},
          eid = {L10},
        pages = {L10},
          doi = {10.1051/0004-6361/201220780},
archivePrefix = {arXiv},
       eprint = {1301.2475},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...550L..10G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


